Repelling-Attracting Hamiltonian Monte Carlo

We propose a variant of Hamiltonian Monte Carlo (HMC), called the Repelling-Attracting Hamiltonian Monte Carlo (RAHMC), for sampling from multimodal distributions. The key idea that underpins RAHMC is a departure from the conservative dynamics of Hamiltonian systems, which form the basis of traditional HMC, and turning instead to the dissipative dynamics of conformal Hamiltonian systems. In particular, RAHMC involves two stages: a mode-repelling stage to encourage the sampler to move away from regions of high probability density; and, a mode-attracting stage, which facilitates the sampler to find and settle near alternative modes. We achieve this by introducing just one additional tuning parameter -- the coefficient of friction. The proposed method adapts to the geometry of the target distribution, e.g., modes and density ridges, and can generate proposals that cross low-probability barriers with little to no computational overhead in comparison to traditional HMC. Notably, RAHMC requires no additional information about the target distribution or memory of previously visited modes. We establish the theoretical basis for RAHMC, and we discuss repelling-attracting extensions to several variants of HMC in literature. Finally, we provide a tuning-free implementation via dual-averaging, and we demonstrate its effectiveness in sampling from, both, multimodal and unimodal distributions in high dimensions.

==> inputs/applications.tex <==
% !TEX root = %WORKSPACE_FOLDER%/plain.tex

\section{Application of Proposed Methodology}
\label{sec:application}


==> inputs/experiments.tex <==
% !TEX root = %WORKSPACE_FOLDER%/plain.tex

\section{Numerical Illustrations}
\label{sec:xperiments}



In the following  examples, we compare auto-tuned \haram{} with four other MCMC methods; HMC that is also equipped with Nesterov's dual averaging, repelling-attracting Metropolis \citep[RAM,][]{tak2018ram},   pseudo-extended HMC \citep[PEHMC,][]{nemeth2019pseudo}, and  wormhole HMC \citep[WHMC,][]{wormhole2014}. 
%\textcolor{red}{We include  HMC as a benchmark to  improve for both unimodal and multimodal cases, RAM as a non-HMC-based multimodal sampler that is competitive in low-dimensional cases,  and both PEHMC and WHMC as HMC-based multimodal samplers that are known to be effective in high dimensions. Not sure what this means?}  
Each MCMC method is implemented for 5,000 iterations with the first 1,000 as burn-in. 

We evaluate their performances based on three metrics: the Wasserstein distance, the average acceptance rate, and the CPU times in seconds. Wasserstein distance is used as a quality measure for the resulting samples. In particular, given two empirical measures $\nu_n$ and $\eta_m$ associated with two samples $\q_1, \ldots, \q_n$ and $\q_1', \ldots, \q_m'$, we use an entropic-regularized version of the Wasserstein distance, called the \textit{Sinkhorn distance} \citep{cuturi2013sinkhorn} to compute $\w(\nu_n, \eta_m)$ and measure the quality of the samples. We refer the readers to \cite{panaretos2019statistical} for a comprehensive introduction to the Wasserstein distance and its applications in statistics.  In addition, we compare auto-correlation functions only in the last example where the target distribution is the multivariate standard  Gaussian distribution. This is because  ACF can be misleading when  a target distribution has multiple modes; the auto-correlation time decreases fast when a Markov chain is stuck at a local mode.  
